Deep Reservoir Computing Using Cellular Automata

Recurrent Neural Networks (RNNs) have been a prominent concept within artificial intelligence. They are inspired by Biological Neural Networks (BNNs) and provide an intuitive and abstract representation of how BNNs work. Derived from the more generic Artificial Neural Networks (ANNs), the recurrent ones are meant to be used for temporal tasks, such as speech recognition, because they are capable of memorizing historic input. However, such networks are very time consuming to train as a result of their inherent nature. Recently, Echo State Networks and Liquid State Machines have been proposed as possible RNN alternatives, under the name of Reservoir Computing (RC). RCs are far more easy to train. In this paper, Cellular Automata are used as reservoir, and are tested on the 5-bit memory task (a well known benchmark within the RC community). The work herein provides a method of mapping binary inputs from the task onto the automata, and a recurrent architecture for handling the sequential aspects of it. Furthermore, a layered (deep) reservoir architecture is proposed. Performances are compared towards earlier work, in addition to its single-layer version. Results show that the single CA reservoir system yields similar results to state-of-the-art work. The system comprised of two layered reservoirs do show a noticeable improvement compared to a single CA reservoir. This indicates potential for further research and provides valuable insight on how to design CA reservoir systems.

==> sections/acknowledgements.tex <==
% use section* for acknowledgment
\section*{Acknowledgments}

I guess that this section depends on the paper standard.

==> sections/background/complexsystems.tex <==
%!TEX root = ../../report.tex

\subsection{Complex Systems}

In the real world, researchers have studied 

Examples of what they are not, are an independent sequence of random numbers, a pendulum, coin tosses.
In general, complex systems are not independent elements.

Emergence

Self-organization


==> sections/background/unconventionalcomputing.tex <==
%!TEX root = ../../report.tex

\subsection{Unconventional computing}

==> tex/customtitle.tex <==
\input{tex/docinfo}

\title{\reportTitle}

\author{\reportAuthor}

\maketitle

\begin{center}
  % {\LARGE \reportTitle}
  % \vspace{\baselineskip}

  % \reportAuthor\\
  \reportAuthorSupplement
\end{center}
